Implementing Efficient Message Logging Protocols as MPI Application Extensions

Message logging protocols are enablers of local rollback, a more efficient alternative to global rollback, for fault tolerant MPI applications. Until now, message logging MPI implementations have incurred the overheads of a redesign and redeployment of an MPI library, as well as continued performance penalties across various kernels. Successful research efforts for message logging implementations do exist, but not a single one of them can be easily deployed today by more than a few experts. In contrast, in this work we build efficient message logging capabilities on top of an MPI library with no message logging capabilities; we do so for two different HPC kernels, one with a global exchange pattern (CG), and one with a neighbourhood exchange pattern (LULESH). While our library of choice ULFM detects failure and recovers MPI communicators, we build on that to then restore the intra- and inter-process data consistency of both applications. This task turns out to be challenging, and we present the methodology for doing so in this work. In the end, we achieve message logging capabilities for each kernel, without the need for an actual message logging runtime underneath. On the performance side, we match state-of-the-art solutions and (a) eliminate event logging and the event logger component altogether, and (b) design a hybrid protocol, which gracefully shifts between global and local rollback, depending on the available payload logging memory. Such a hybrid protocol between local and global rollback has not been previously proposed to our knowledge. Our extensions span a few hundred lines of code for each kernel, are open-sourced, and enable local and global rollback after process failure.

==> correctness.tex <==
\subsection{Correctness}

Validating the correctness of the proposed algorithm is essential.
There are two different correctness aspects to verify:

\subsubsection{Does the modified kernel behave as a local rollback, instead of global rollback?}

%For the first question, one simple measure we use is the aggregated total number of iterations across all processes to complete a benchmark.
%In the proposed protocol, only failed processes roll back to a checkpoint, so less iterations should be required for survivor processes.

The choice of failure scenarios is significantly more difficult to make, due to the extensive nature of possible settings. We opt for a few clearly defined and reproducible experiments here.
\begin{itemize}
\item First, we terminate a fixed process at 4 different phases of the same iteration.
\item Then, we terminate fixed processes at different iterations.
\end{itemize}

We first terminate a fixed process in a fixed post-backup iteration, during any of 4 compute phases, which were earlier outlined in blue in Fig. \ref{cg:phases}.
As shown in Tab. \ref{tab:kill-in-phases}, every change in the crash phase, even in the same iteration, leads to differences in when the processes detect the failure.
Each of these differences is handled differently by the replay protocol.

\begin{table}
\begin{tabular}{|p{1cm}|p{1cm}|p{1cm}|p{4cm}|}
rank killed & phase killed & iteration killed & failure detected by survivors in iter? \\
\hline
2  & 1 & 20 & all in iter 20 \\
\hline
2 & 2 & 20 & first 8 in iter 20, remaining in iter 21 \\
\hline
2 & 3 & 20 & first 8 in iter 20, remaining in iter 21 \\
\hline
2 & 4 & 20 & all in iter 21 \\  
\hline
\end{tabular}
\caption{Consistency issues detailed in Sect. \ref{sec:replay-mpi} manifest differently based on the failure phase within an iteration. Benchmark used: cg.C with 64 processes.}
\label{tab:kill-in-phases}
\end{table}

We then incrementally increase the iteration of failure after the last global checkpoint, ranging from 1 to 20 (a NAS CG iteration is set to a maximum of 25).
No process needs to roll back further than this last global checkpoint, whether we employ global or local rollback.
We crash arbitrary, but fixed, processes: here, we choose rank 0 for the single-process crash scenario, and ranks 0 and 8 for the double-crash scenarios.
The total of recomputed iterations are shown (in logarithmic scale) in Fig. \ref{fig:local-vs-global}.
Global rollback leads to all processes rolling back, both for single and double-crash scenarios.
For local rollback, only the failed process needs to roll back -- for double-crashes, this doubles the repeated iterations.
Overall, local rollback only repeats the iterations of the failed process, compared to global rollback, which rolls back every process.
This is the expected behaviour of any local rollback strategy. 

\begin{figure}
\includegraphics[width=0.45\textwidth]{data/class-C/64/failures}
\caption{Total of recomputed iterations for local and global rollback when triggering single or double-crash for processes ranging from 1 to 20 iterations after a checkpoint; the used benchmark is cg.C with 64 processes.}
\label{fig:local-vs-global}
\end{figure}

\subsubsection{Is the algorithm still correct?}

This question can be answered with the support of the validation mechanisms already in place in the NAS benchmarks.
The CG benchmark provides a fixed zeta value to compare against, which is invaluable as a correctness measure during the design of local rollback.



==> ft-cg.tex <==

% !TEX root = paper.tex

 \begin{algorithm}
 %\algnewcommand{\IIf}[1]{\State\algorithmicif\ #1\ \algorithmicthen}
  %\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}
     \begin{algorithmic}[1]
      { \color{blue}
     	\Function{send}{m,p,i}
	\If {($peer\_iter(p) \leq i$)}
	%\If {($i  \bmod CP\_INT < LOG\_SIZE$)}
	\State \Call{Append}{buffer($i \bmod CP\_INT$), m}
	%\Comment non-blocking!
	%\EndIf
	\State \Call{psend}{m,p}
	\EndIf
	\EndFunction
	}
         \Function{CG}{}
         \State \dots
         \For {$i \in1 \dots niter$}
         \For{$p \in reduce\_neighbours$} \Comment $q \gets A.p$ Part 1
         \State \Call{Irecv}{q,p}
        { \State \color{blue}  \Call{send}{w,p,i}}
         \State \Call{wait}{}
         \EndFor
	\State \dots
	 \State $p \gets $ transpose process
         \If {(p $\neq$ me)} \Comment $q \gets A.p $ Part 2
         \State \Call{Irecv}{q,p}
         {\State \color{blue} \Call{send}{w,p,i}}
         \State \Call{wait}{}
         \EndIf
	\State \dots
         \For{$p \in reduce\_neighbours$} \Comment obtain $d$
          \State \Call{Irecv}{d,p}
          {\State \color{blue} \Call{send}{sum,p,i}}
          \State \Call{wait}{}
         \EndFor
	\State \dots
         \For{$p \in reduce\_neighbours$} \Comment obtain $rho$
         \State \Call{Irecv}{rho,p}
         {\State \color{blue} \Call{send}{sum,p,i}}
         \State \Call{wait}{}
	 \State \dots
         \EndFor
	\State \dots
	{\color{blue}
	\If {($i \bmod CP\_INT = 0$)}
	 \label{line:cp}
	\State checkpoint iter $i$
	%\Comment blocking!
	\EndIf
         \EndFor
         }
         \State \dots
         \EndFunction
     \end{algorithmic}
     \caption{An outline of the original communication pattern in the CG loop (in black), and the extensions enabling checkpointing state and message contents (in blue).}
     \label{alg:cg}
 \end{algorithm}


==> replay-code.tex <==
% !TEX root = paper.tex

 \begin{algorithm}
     \begin{algorithmic}
         {\color{blue}
         \Function{GlobalOrLocal}{}
          \State $ peer\_iter \gets allgather \dots$
          \If {$me = restarted$}
            \State \Call{Read global cp}{}
          \Else
           \State $ maxit \gets  max(peer\_iter)$
           \State $ minit \gets  min(peer\_iter)$
          \If {$(maxit \bmod CP\_INT < LOG\_SIZE)$}
          \label{alg:check-g-or-l}

         \ForAll{$it = minit \dots maxit$}
                  \label{alg:replay-start}
         \For{s $\in$ sequence of send calls in CG iter $it$}
         \State $peer \gets $ receiver of operation s
         \If {$peer\_iter(peer) < peer\_iter(me)$}
            \State \Call{send}{buffer($it \bmod CP\_INT$),peer} 
         \EndIf
         \EndFor
         \EndFor
         \label{alg:replay-end}
          \Else
          \State \Call{Read global cp}{}
          \EndIf
          \EndIf
            \State \Call{CG}{}
         \EndFunction{}
         }
              \caption{Local rollback algorithm: The survivors replay message logs similarly to message logging MPI implementations.}
     \label{alg:replay}
     \end{algorithmic}    
 \end{algorithm}


==> table-live-updates.tex <==
% !TEX root = paper.tex


\begin{table}
\small{
\begin{tabular}{|p{1cm}|p{3cm}|p{3cm}|}
& message sequence & live history \\
\hline
Failed - restarted process (rank 2) & 
$(1,sendrecv^{(4,10)}_3)$, 
%checkpoint,
{
\color{red}
$(1,sendrecv^{(1,11)}_0)$, 
\dots,
$(1,sendrecv^{(2,13)}_8)$, 
%crash and restart, 
}
{
\color{blue}
$(2,recv^{(1,11)}_0)$,
$(2,recv^{(1,11)}_3)$,
\dots
}
$(2,sendrecv^{0,13}_0)$
&
$(1,sendrecv^{(4,10)}_3)$, 
$(1,send^{(1,11)}_0)$, 
\dots,
$(1,send^{(2,13)}_8)$, 
\dots,
$(2,recv^{(1,11)}_0)$,
$(2,recv^{(1,11)}_3)$,
$(2,sendrecv^{0,13}_0)$
 \\
 \hline
% survivor (rank 3) &
% $\dots$, $(1,sendrecv^{(4,10)}_3)$, $(2,sendrecv^{(2,11)}_0)$, $\dots$.
% \\
% \hline
 survivor (rank 3)  &
 $(1,sendrecv^{(4,10)}_2)$,
{
\color{red}
 $(1,sendrecv^{(1,11)}_1)$,
\dots,
$(1,sendrecv^{(3,13)}_2)$,
%$(1,sendrecv^{(3,11)}_2)$,
}
%detect failure,
{
\color{blue}
$(2,send^{(1,11)}_2)$,
$(2,send^{(2,11)}_2)$,
\dots,
}
$(2,sendrecv^{(1,13)}_1)$
&

 $(1,sendrecv^{(4,10)}_2)$,
 $(1,recv^{(1,11)}_1)$,
\dots,
$(1,recv^{(3,13)}_2)$,
$(2,send^{(1,11)}_2)$,
$(2,send^{(2,11)}_2)$,
$(2,sendrecv^{(1,13)}_1)$
 \\
\hline
\end{tabular}
}
\caption{Left column: Message events for ranks 2 and 3 of the failure scenario of Fig. \ref{fig:failure-scenario}.
Unaffected messages are shown in black. Lost message events are shown in red. Events relating to replay are shown in blue.
Right column: live history of message events, which excludes lost events, for ranks 2 and 3 and same scenario.
}
\label{tab:live-history}
\end{table}

